MobileH2R: Learning Generalizable Human to Mobile Robot Handover Exclusively from Scalable and Diverse Synthetic Data

This paper introduces MobileH2R, a framework for learning generalizable vision-based human-to-mobile-robot (H2MR) handover skills. Unlike traditional fixed-base handovers, this task requires a mobile robot to reliably receive objects in a large workspace enabled by its mobility. Our key insight is that generalizable handover skills can be developed in simulators using high-quality synthetic data, without the need for real-world demonstrations. To achieve this, we propose a scalable pipeline for generating diverse synthetic full-body human motion data, an automated method for creating safe and imitation-friendly demonstrations, and an efficient 4D imitation learning method for distilling large-scale demonstrations into closed-loop policies with base-arm coordination. Experimental evaluations in both simulators and the real world show significant improvements (at least +15% success rate) over baseline methods in all cases. Experiments also validate that large-scale and diverse synthetic data greatly enhances robot learning, highlighting our scalable framework.

==> table/table_for_ppt.tex <==


% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{3mm}
% \small
% \begin{tabular}{cccc}
% \hline
% \textbf{Num. of Demos / training set}              & m0 & n0 &  s0\\ \hline
% 10k, n0  & 53.4 & 63.8 & 77.8\\
% 100k, n0            &          &        &    \\
% 1k, n0          & & & \\
% 10k, m0          & 45.3 & 62.0 & 76.4 \\
% 10k, s0         & 22.0 & 35.3 &  34.0      \\

% \end{tabular}
% \vspace{-1mm}
% \caption{\textbf{Evaluation on Varying demonstration numbers and Assets.} We compare the policy's performance across three testing sets, examining the impact of different demonstration numbers and asset variations on the success rate.}
%  \vspace{-1em}
%  \label{tab:scaling}
% \end{table}
\definecolor{darkbrown}{RGB}{120, 60, 30}
\definecolor{deepolivegreen}{RGB}{85, 107, 47}
\definecolor{green}{RGB}{0, 255, 0}
% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{3mm}
% \small
% \begin{tabular}{cccc}
% \hline
% \textbf{Num. of Demos / training set}              & m0 & n0 &  s0\\ \hline
% 100k, n0            &          &        &    \\
% 1k, n0          & & & \\
% 10k, n0  & 53.4 & 63.8 & 77.8\\
% 10k, m0          & 45.3$\downarrow$ & 62.0 & 76.4 \\
% 10k, s0         & 22.0 & 35.3 &  34.0      \\
% \end{tabular}
% \vspace{-1mm}

% % Draw braces using TikZ
% \begin{tikzpicture}[overlay, remember picture]
%     % Red curly brace for the first three rows (corrected direction)
%     \draw[decorate, decoration={brace, amplitude=6pt}, color={rgb,255:red,120; green,60; blue,30}, thick] 
%         ([yshift=-6pt] -2.4, 0.95) -- ([yshift=6pt] -2.4, 1.60) 
%         node[midway, xshift=-0.5cm, red] {};
%     % Blue curly brace for the last two rows (aligned precisely)
%     \draw[decorate, decoration={brace, amplitude=6pt}, color={rgb,255:red,85; green,107; blue,47}, thick] 
%         ([yshift=-6pt] -2.7, 0.15) -- ([yshift=6pt] -2.7, 0.8) 
%         node[midway, xshift=-0.5cm, blue] {};
% \end{tikzpicture}

% \caption{\textbf{Evaluation on Varying demonstration numbers and Assets.} We compare the policy's success rate across three testing sets, examining the impact of different demonstration numbers within \textcolor{darkbrown}{brown braces} and asset variations within \textcolor{deepolivegreen}{green braces}.}
%  \vspace{-1em}
%  \label{tab:scaling}
% \end{table}



% \definecolor{darkbrown}{RGB}{120, 60, 30}
% \definecolor{deepolivegreen}{RGB}{85, 107, 47}

% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{3mm}
% \small
% \begin{tabular}{cccc}
% \hline
% \textbf{Num. of Demos / training set}              & m0 & n0 &  s0\\ \hline
% 1k, n0          & 53.4 & 42.3 & 57.6 \\
% 10k, n0   & 63.8 & 53.4  & 77.8\\
% 100k, n0            &  65.6     &   56.6     &  82.6  \\

% % 10k, m0          &  62.0 & 45.3 & 76.4 \\
% % 10k, s0          & 35.3  & 22.0 &  34.0      \\
% \hline
% \end{tabular}
% \vspace{-1mm}

% \caption{\textbf{Evaluation on varying demonstration numbers and Assets.} We compare the policy's success rate across three testing sets, examining the impact of different demonstration sizes within \textcolor{darkbrown}{brown braces} and asset variations within \textcolor{deepolivegreen}{green braces}.}
%  \vspace{-1em}
%  \label{tab:ppt1}
% \end{table}



% \begin{table}[t]
% \centering
% \setlength{\tabcolsep}{3mm}
% \small
% \begin{tabular}{cccc}
% \hline
% \textbf{Num. of Demos / training set}              & m0 & n0 &  s0\\ \hline
% 10k, m0 (simple synthetic data)         &  62.0 & 45.3 & 76.4 \\
% 10k, s0 (real-world mocap data)         & 35.3  & 22.0 &  34.0      \\
% 10k, n0 (complex synthetic data)  & 63.8 & 53.4  & 77.8\\
% \hline
% \end{tabular}
% \vspace{-1mm}

% \caption{\textbf{Evaluation on varying demonstration numbers and Assets.} We compare the policy's success rate across three testing sets, examining the impact of different demonstration sizes within \textcolor{darkbrown}{brown braces} and asset variations within \textcolor{deepolivegreen}{green braces}.}
%  \vspace{-1em}
%  \label{tab:ppt1}
% \end{table}


\begin{table}[t]
\centering
\setlength{\tabcolsep}{3mm}
\small
\begin{tabular}{cccc}
\hline
\textbf{Demo strategies}              & m0 & n0 &  s0\\ \hline
w/o future obstacle avoidance           & 58.7   & 48.5 &  75.7  \\
w/o final pose constraints & 58.4  & 43.2 & 69.4 \\
Ours   &\textbf{ 63.8} & \textbf{53.4} & \textbf{77.8}\\
\hline
\end{tabular}
\vspace{-1mm}
\caption{\textbf{Evaluation on different demonstration generation strategies.} We compare the policy's success rate across three testing sets. They all trained on ``n0''.}
 \vspace{-1em}
 \label{tab:demo_method_ppt}
\end{table}


\begin{table}[t]
\centering
\setlength{\tabcolsep}{3mm}
\small
\begin{tabular}{cccc}
\hline
\textbf{Demo strategies}              & m0 & n0 &  s0\\ \hline
w/o imitation-friendly loss          & 56.8  & 46.4 & 56.9 \\
Ours   &\textbf{ 63.8} & \textbf{53.4} & \textbf{77.8}\\
\hline
\end{tabular}
\vspace{-1mm}
\caption{\textbf{Evaluation on different demonstration generation strategies.} We compare the policy's success rate across three testing sets. They all trained on ``n0''.}
 \vspace{-1em}
 \label{tab:demo_method_ppt2}
\end{table}
